Variational Relational Point Completion Network

Real-scanned point clouds are often incomplete due to viewpoint, occlusion, and noise. Existing point cloud completion methods tend to generate global shape skeletons and hence lack fine local details. Furthermore, they mostly learn a deterministic partial-to-complete mapping, but overlook structural relations in man-made objects. To tackle these challenges, this paper proposes a variational framework, Variational Relational point Completion network (VRCNet) with two appealing properties: 1) Probabilistic Modeling. In particular, we propose a dual-path architecture to enable principled probabilistic modeling across partial and complete clouds. One path consumes complete point clouds for reconstruction by learning a point VAE. The other path generates complete shapes for partial point clouds, whose embedded distribution is guided by distribution obtained from the reconstruction path during training. 2) Relational Enhancement. Specifically, we carefully design point self-attention kernel and point selective kernel module to exploit relational point features, which refines local shape details conditioned on the coarse completion. In addition, we contribute a multi-view partial point cloud dataset (MVP dataset) containing over 100,000 high-quality scans, which renders partial 3D shapes from 26 uniformly distributed camera poses for each 3D CAD model. Extensive experiments demonstrate that VRCNet outperforms state-of-theart methods on all standard point cloud completion benchmarks. Notably, VRCNet shows great generalizability and robustness on real-world point cloud scans.

==> figure/gt_partial.tex <==
% \begin{figure}
%     \centering
%     \subfigure[]{
%     \includegraphics[width=1\linewidth]{src/partial.pdf}
%     \label{fig:MVP_a}
%     }
%     % \hspace{.0275\linewidth}
%     \subfigure[]{
%     \includegraphics[width=1\linewidth]{src/gt.pdf}
%     \label{fig:MVP_b}
%     }
%     \caption{Caption}
%     \label{fig:MVP}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{src/gt_partial.pdf}
    \vspace{-0.85cm}
    \caption{(a) Comparison for rendered partial point clouds with different camera resolutions. (b) Comparison for sampled point clouds using Uniformly Sampling and Poisson Disk Sampling.}
    \label{fig:mvp}
\end{figure}

==> figure/mv_dataset.tex <==
\begin{figure}
    \centering
    \subfigure[]{
    \includegraphics[width=.2\linewidth]{src/camera_pose_ring.pdf}
    }
    \hspace{.0275\linewidth}
    \subfigure[]{
    \includegraphics[width=.65\linewidth]{src/mv_airplane.pdf}
    }
    % \subfigure[]{
    % \includegraphics[width=.3\linewidth]{src/psak.pdf}
    % }
    % \includegraphics[width=1\linewidth]{src/mv_airplane.pdf}
    \vspace{-0.4cm}
    \caption{An example for 26 partial observations of a complete CAD model. (a) shows our uniformly distributed camera poses (each blue dot denotes a camera location that looks towards the centre of the sphere), and (b) shows all the rendered partial point clouds by the 26 camera poses.}
    \label{fig:mv_dataset}
\end{figure}

==> figure/mv_qua.tex <==
\begin{figure}
    \centering
    % \includegraphics[width=1\linewidth]{src/mv_qua_update.pdf}
    % \includegraphics[width=1\linewidth]{src/mv_qua_update_body.pdf}
    \includegraphics[width=1\linewidth]{src/mv_qua_v2.pdf}
    \vspace{-8mm}
    \caption{\textbf{Our completion results conditioned on different partial observations.} The arrows indicate the viewing angles. In (a) and (b), two knots can be partially observed for the pole of the lamp, and hence we can generate two complete knots in the complete shapes. In (c), only 1 knot is observed, and then we reconstruct 1 complete knot. If no knots are observed (see (d)), our \OM{} will generate a smooth pole without knots.
    % , as shown in (d).
    }
    \label{fig:mv_qua}
\end{figure}


% \begin{figure*}
%     \centering
%     % \includegraphics[width=1\linewidth]{src/mv_qua_update.pdf}
%     % \includegraphics[width=1\linewidth]{src/mv_qua_update_body.pdf}
%     \includegraphics[width=0.85\linewidth]{src/mv_qua_hori_update.pdf}
%     \vspace{-4mm}
%     \caption{\textbf{Our completion results conditioned on different partial observations.} In (a) and (b), two knots can be partially observed for the pole of the lamp, and hence we can generate two complete knots. In (c), only 1 knot is observed, and then we reconstruct 1 complete knot. If no knots are observed (see (d)), our \OM{} will generate a smooth pole without knots.
%     % , as shown in (d).
%     }
%     \label{fig:mv_qua}
% \end{figure*}

